Assessing Agile Transformation Success Factors

Research on success factors involved in the agile transformation process is not conclusive and there is still need for guidelines to help in the transformation process considering the organizational context (culture, values, needs, reality and goals). The usage of success factors as a tool to help agile adoption raises the following research question: What are the success factors for an organization and their teams in preparation for the agile transformation process? This research presents an assessment of the organizational environment including the company's goals and the perception of the team members to provide awareness of how the organization should prepare for the next steps in the agile transformation. The findings show that a company based in Chicago, USA, succeeded implementing customer involvement and self-organized teams but faces challenges with measurement models and training. The main contribution of the research is understand which success factors exist in their environment and how they can be used during agile adoption.

==> background.tex <==
\section{Agile Transformation Success Factor}
\label{sec:Background}

Agile transformation process (ATP) is the process of transforming an organization into agile~\cite{Gandomani2014exploring}. This process impacts all areas of the organizations. People are required to change their mindset and behavior~\cite{gandomani2014human, Conboy2010People}, they need to modify the way they work as a team. Processes are affected and need to be adjusted, management style and attitudes are affected as well~\cite{Gandomani2014exploring}.The agile transition also involves technical transformation~\cite{GandomaniZGSS13}.

It is important that organizations understand the reach of the changes involved in ATP. It helps to create the awareness needed for this type of initiative, prepares the team for the upcoming challenges and increases the chances of achieving the proposed goals~\cite{TaylorGCMK08, Gandomani2014exploring}. Further, organizations need to control effort and costs associated with ATP~\cite{GandomaniZGSS14}. In some cases, companies might not survive to a failed adoption attempt or the improvement initiatives might stop at once~\cite{TaylorGCMK08}.

%\subsection{Agile Transformation Success Factors}

Researchers have been studied agile transformation success factors in the search for paths that enable organizations to have control over their adoption process and to be able to deal with known barriers and challenges during the implementation~\cite{GandomaniZGSS14}.

Some researchers refer to the success factors as challenges for agile adoption ~\cite{NerurMM05,Conboy2010People,gregory2015agile} but it is basically a different view of the same factor. All researches we found on this topic are concerned about detecting which factors organizations must evaluate when conducting ATPs to achieve success. 

Examples of success factors are: customer involvement~\cite{ChowC08}, distributed power to make decisions~\cite{gandomani2013obstacles}, involved leadership~\cite{TaylorGCMK08}, management style~\cite{NerurMM05}, knowledge sharing~\cite{srinivasan2009organizational}, commitment/engagement~\cite{gregory2015agile}, the need to understand and learn values and principles of agile, not just the practices~\cite{Conboy2010People}, lack of training (we used need of training in our research)~\cite{gandomani2014human}, trust~\cite{gregory2015agile}, team members buy-in~\cite{Gandomani2014exploring} and teamwork~\cite{chan2009acceptance}.



==> limitations.tex <==
\subsection{Limitations}
\label{sec:Limitations}

The limitations of this research are the small dataset for the application of the Rasch algorithm and a single company validation of the assessment. 

Even though the we followed the guidelines provided by Lahrmann \textit{et al.}~\cite{Lahrmann2011} and the fit statistics of the Rasch algorithm are considered good, there is still a chance of bias because of the usage of a dataset composed of 14 respondents. We are working on a survey using the assessment to gather data from multiple companies.

Another risk of bias involves the validation of the assessment by a single company. This could create distortions on the assessment in case the analyzed company operates in a very different way from other companies using agile methods and practices. To address this risk, we are planning new case studies using the assessment for feedback and improvement.



==> related-work.tex <==
\section{Background}
\label{sec:Background}

%%%%%%%%%%
\subsection{Agile Transformation Success Factor}
%%%%%%%%%%

Agile transformation process (ATP) is the process of transforming an organization into agile~\cite{Gandomani2014exploring}. This process impacts all areas of the organizations. People are required to change their mindset and behavior~\cite{gandomani2014human, Conboy2010People}, they need to modify the way they work as a team. Processes are affected and need to be adjusted, management style and attitudes are affected as well~\cite{Gandomani2014exploring}.The agile transition also involves technical transformation~\cite{GandomaniZGSS13}.

It is important that organizations understand the reach of the changes involved in ATP. It helps to create the awareness needed for this type of initiative, prepares the team for the upcoming challenges and increases the chances of achieving the proposed goals~\cite{TaylorGCMK08, Gandomani2014exploring}. Further, organizations need to control effort and costs associated with ATP~\cite{GandomaniZGSS14}. In some cases, companies might not survive to a failed adoption attempt or the improvement initiatives might stop at once~\cite{TaylorGCMK08}.

%\subsection{Agile Transformation Success Factors}

Agile transformation success factors have been studied by researchers to point paths to allow organizations to have control over their adoption process and to be able to deal with known barriers and challenges during the implementation~\cite{GandomaniZGSS14}.

Some researchers refer to the success factors as challenges for agile adoption ~\cite{NerurMM05,Conboy2010People,gregory2015agile} but it is a different view of the same factor. All researches we found on this topic are concerned about detecting which factors should be evaluated by organizations when conducting ATPs to achieve success. 

Examples of success factors are: customer involvement~\cite{ChowC08}, distributed power to make decisions~\cite{gandomani2013obstacles}, involved leadership~\cite{TaylorGCMK08}, management style~\cite{NerurMM05}, knowledge sharing~\cite{srinivasan2009organizational}, commitment/engagement~\cite{gregory2015agile}, the need to understand and learn values and principles of agile, not just the practices~\cite{Conboy2010People}, lack of training (we used need of training in our research)~\cite{gandomani2014human}, trust~\cite{gregory2015agile}, team members buy-in~\cite{Gandomani2014exploring} and teamwork~\cite{chan2009acceptance}.

%%%%%%%%%%
\subsection{Related Work}
\label{sec:RelatedWork}
%%%%%%%%%%

Taylor \textit{et al.}~\cite{TaylorGCMK08} proposed intrusive risk assessment to prepare small companies to adopt agile methods. The articles express concerns about the capability of small companies to survive to a failed agile adoption attempt and proposes the assessment to point directions if the organization should pursue the agile adoption or use a traditional approach for software development. This assessment can provide a direction on agile adoption per project basis. The authors used the agility/discipline assessment (ADA) developed by Boehm and Tuner~\cite{boehm2003using} and they applied it to six organizations proposing adaptations to each of the contexts. The areas contemplated by the assessment were criticality, personnel, dynamism, culture, client involvement and team distribution. 

The assessment proposed by Taylor \textit{et al.}~\cite{TaylorGCMK08} has similarities to our work: it is used to evaluates the risks of agile adoption, its goal is to involve the team members in the discussion around agile adoption and it requires a minimum overhead. The work of Taylor \textit{et al.}~\cite{TaylorGCMK08}  focuses on the choice between agile and traditional approaches at the project level while our assessment is focused on the preparation for an ATP and discovery of the current state of the agile success factors at the organization level. Their assessment considers different aspects from the ones considered in our assessment: criticality, personnel, dynamism, culture, client involvement and team distribution. Our assessment considers broader aspects of the organization such as management style, team behavior and relationship, and processes.

%The criticality aspect considers the loss due to defects in the software. This is related to .

%The personnel aspect takes into account - it is known that agile methods require experienced people to work on 

%Dynamism is an aspect that can be considered 

%Team distribution

Gandomani \textit{et al.}~\cite{gandomani2013obstacles} provided a comparison between traditional and agile software development methods and the challenges of transitioning to agile methods. They classify the challenges for agile transition into four categories: organization and management; people; process; technology and tools. Their work also highlighted that this process affects the whole organization. A strong message from their study is that all members should be involved to deal with such challenges. This part of their work is similar to ours up to the point of the proposed success factors groups. The groups are similar between the two researches but we have aggregated terms from different references. However, their work stops at this point while, in our research, the success factors groups are used as basis for the agile transformation success factors assessment definition. We understand that our research has a practice oriented goal with the assessment proposal and validation.


Gregory \textit{et al.}~\cite{gregory2015agile} analyzed the shift between agile adoption challenges as the adoption levels and the state of practice evolved over the years. They collected agile challenges during conferences in the years of 2013 and 2014 and conducted a thematic analysis. They organized the challenges into categories: organization, sustainability,
culture, teams, scale, value and, claims and limitations. Their conclusion on the evolution of the agile adoption challenges is that:

\begin{itemize}
	\item Some challenges have persisted in the literature for many years and are hard to address.
	\item Other have persisted over the years but with a shift in the focus (scaling and distributed teams for instance).
	\item Some challenges have not gained attention as sustainability, business engagement, failure and limitations.
	\item There are challenges addresses by academic researches but remains considered as a challenge by organizations and practitioners.
\end{itemize}

Gregory \textit{et al.}~\cite{gregory2015agile} presented an interesting analysis of agile challenges between practice and literature points of view. They gathered their main dataset from practitioners, defined themes and sub-themes, and compared their findings to references in the literature. Their work on the themes and sub-themes creation is similar to the work we have done on the success factors groups definition even though the groups are not similar. The differences between the researches are that their final findings are the analysis of the evolution of the agile challenges over time that can be used for action researches as a starting point. In our case, we are introducing a practical approach to use the proposed agile transformation success factor groups in the format of an assessment. 


Chow and Cao~\cite{ChowC08} investigated the critical success factors in agile methods adoption and proposed groups to classify critical success factors and created a model to validate how the critical success factors affects the quality, cost, scope and time of agile software development projects. The groups of factors were defined as organizational, people, process, technical and project. They conducted a survey to validate hypothesis for each of the success factors and analyzed the correlation between success factors and project success to establish critical success factors. The critical success factors according to their results are: delivery strategy, agile software engineering techniques and high qualified team. They also found three factors the can be considered certain success factors: good agile project management process, agile-friendly team environment and strong customer involvement.

The similarities between their research and ours is on the definition of the success factors groups approach and on the usage of statistical methods to validate the gathered data. The differences are the usage of case study to gather data and to validate the assessment in our study. The final product of the researches are different as well. Chow and Cao's work~\cite{ChowC08} produced a model to associate success factors to software development projects aspects, meanwhile our work resulted in the agile transformation success factors assessment.

